3D-SIS: 3D Semantic Instance Segmentation of RGB-D Scans

We introduce 3D-SIS, a novel neural network architecture for 3D semantic instance segmentation in commodity RGB-D scans. The core idea of our method is to jointly learn from both geometric and color signal, thus enabling accurate instance predictions. Rather than operate solely on 2D frames, we observe that most computer vision applications have multi-view RGB-D input available, which we leverage to construct an approach for 3D instance segmentation that effectively fuses together these multi-modal inputs. Our network leverages high-resolution RGB input by associating 2D images with the volumetric grid based on the pose alignment of the 3D reconstruction. For each image, we first extract 2D features for each pixel with a series of 2D convolutions; we then backproject the resulting feature vector to the associated voxel in the 3D grid. This combination of 2D and 3D feature learning allows significantly higher accuracy object detection and instance segmentation than state-of-the-art alternatives. We show results on both synthetic and real-world public benchmarks, achieving an improvement in mAP of over 13 on real-world data.

==> sections/8limitations.tex <==
\section{Limitations}
While our 3D instance segmentation approach leveraging joint color-geometry feature learning achieves marked performance gain over state of the art, there are still several important limitations.
%
For instance, our current 3D bounding box predictions are axis-aligned to the grid space of the 3D environment. 
Generally, it would be beneficial to additionally regress the orientation for object instances;  e.g., in the form of a rotation angle.
Note that this would need to account for symmetric objects where poses might be ambiguous.
%
At the moment, our focus is also largely on indoor environments as we use commodity RGB-D data such as a Kinect or Structure Sensor. 
However, we believe that the idea of taking multi-view RGB-D input is agnostic to this specific setting; for instance, we could very well see applications in automotive settings with LIDAR and panorama data.
%
Another limitation of our approach is the focus on static scenes.
Ultimately, the goal is to handle dynamic or at least semi-dynamic scenes where objects are moving, which we would want to track over time.
Here, we see a significant research opportunities and a strong correlation to tracking and localization methods that would benefit from semantic 3D segmentation priors.
